MultiEM: Efficient and Effective Unsupervised Multi-Table Entity Matching

Entity Matching (EM), which aims to identify all entity pairs referring to the same real-world entity from relational tables, is one of the most important tasks in real-world data management systems. Due to the labeling process of EM being extremely labor-intensive, unsupervised EM is more applicable than supervised EM in practical scenarios. Traditional unsupervised EM assumes that all entities come from two tables; however, it is more common to match entities from multiple tables in practical applications, that is, multi-table entity matching (multi-table EM). Unfortunately, effective and efficient unsupervised multi-table EM remains under-explored. To fill this gap, this paper formally studies the problem of unsupervised multi-table entity matching and proposes an effective and efficient solution, termed as MultiEM. MultiEM is a parallelable pipeline of enhanced entity representation, table-wise hierarchical merging, and density-based pruning. Extensive experimental results on six real-world benchmark datasets demonstrate the superiority of MultiEM in terms of effectiveness and efficiency.

==> proofs.tex <==
\section{Proofs}
\label{proof}

\subsection{Proof of Lemma \ref{lemma:pairwise_matching}}
\label{proof:pairwise_matching}

For pairwise matching of $S$ tables, $\tbinom{S}{2}$ times of two-table EM methods are applied. Therefore, its complexity depends on the complexity of the applied two-table EM method, denoted as:

\begin{equation}
    T_{p}(S,n)=O(S^2 f(n))
\end{equation}
Here, $f(n)$ is the complexity of matching two tables.

Suppose that the mutual top-K search (i.e., with complexity $O(2kn\log n)$) is applied to match two tables. Therefore, the overall complexity of pairwise matching is computed as:

\begin{equation}
    T_{p}(S,n)=O(S^2 2kn\log n)
\end{equation}

For other more complex EM methods \cite{li2020deep,wang2022promptem,li2021auto,tu2022domain}, $f(n)$ is much higher than $O(2kn\log n)$, so the overall complexity: 

\begin{equation}
    T_{p}(S,n) \geq O(S^2 2kn\log n)
\end{equation}

\subsection{Proof of Lemma \ref{lemma:chain_matching}}
\label{proof:chain_matching}

For chain matching of $S$ tables, first, the base table is selected, and then the other $S-1$ tables are matched one by one. We refer the above $f(n)$ as the matching complexity of two tables. Here, $f(n)=O(kn\log n^{\prime}+kn^{\prime}\log n)$ because the sizes of the two tables are different. As matching, the unmatched entities are retained, leading to an increase in the size of the base table. Therefore, the overall complexity:

\begin{equation}
    \begin{split}
        T_c(S,n)& = \sum_{i=1}^{S-1} O(kin\log n+kn\log in) \\ 
        &=\sum_{i=1}^{S-1} O(kin\log n) + \sum_{i=1}^{S-1} O(kn\log in) \\ 
        &=O(kn(\sum_{i=1}^{S-1}i \log n+\sum_{i=1}^{S-1}\log n+\sum_{i=1}^{S-1}\log i)) \\
        &=O(S^2kn\log n)+ O(Skn\log n)+ O(kn\sum_{i=1}^{S-1}\log i) \\
        &\geq O(S^2kn\log n)
    \end{split}
\end{equation}

\subsection{Proof of Lemma \ref{lemma:hierarchical_merging}}
\label{proof:hierarchical_merging}

For each hierarchy $i$ from 1 to $\log S$ with $\frac{S}{2^{i-1}}$ tables, we apply the two-table merging function (i.e., Algorithm \ref{algo:merging_two_tables}) to every two tables. Therefore, the time complexity can be expressed as:

\begin{equation}
    T(S,n)=\sum_{i=1}^{\log S} \frac{S}{2^{i}} t(i)
\end{equation}
Here, $t(i)$ denotes the complexity of merging two tables at hierarchy $i$, that is, $t(i)=O(2kn^{\prime}\log n^{\prime})$, where $n'$ is the size of the tables at this hierarchy.

To be more specific, for two tables of size $n$, the size of the merged table $n^{\prime}<=2n$. In conclusion, the final time complexity can be calculated as follows:

\begin{equation}
    \begin{split}
        T(S,n)& \leq \sum_{i=1}^{\log S} \frac{S}{2^{i}} O(2k2^{i-1}n\log (2^{i-1}n))  \\
        & \leq O(Skn \sum_{i=1}^{\log S} \log (2^{i-1}n)) \\
        & \leq O(Skn (\sum_{i=1}^{\log S} \log 2^{i-1} + \sum_{i=1}^{\log S} \log n)) \\
        & \leq O(Skn (\log S \frac{\log S -1}{2} +\log S \log n)) \\
        & \leq O(Skn \log S (\frac{\log S -1}{2}+\log n))
    \end{split}
\end{equation}

Since $S \ll n$ in almost all cases, the complexity can be expressed as $O(Skn \log S \log n)$
